Scalable Ray Tracing Using the Distributed FrameBuffer

Image- and data-parallel rendering across multiple nodes on high-performance computing systems is widely used in visualization to provide higher frame rates, support large data sets, and render data in situ. Specifically for in situ visualization, reducing bottlenecks incurred by the visualization and compositing is of key concern to reduce the overall simulation runtime. Moreover, prior algorithms have been designed to support either image- or data-parallel rendering and impose restrictions on the data distribution, requiring different implementations for each configuration. In this paper, we introduce the Distributed FrameBuffer, an asynchronous image-processing framework for multi-node rendering. We demonstrate that our approach achieves performance superior to the state of the art for common use cases, while providing the flexibility to support a wide range of parallel rendering algorithms and data distributions. By building on this framework, we extend the open-source ray tracing library OSPRay with a data-distributed API, enabling its use in data-distributed and in situ visualization applications.

==> Makefile <==
all: paper summary_of_changes.pdf

CONTENT=distrib-ospray
BIBLIOGRAPHY=$(wildcard *.bib)
ALLTEXFILES=$(wildcard *.tex content/*.tex)
ALLFIGS=$(wildcard png/* figures/* *.bib)
LATEX_ARGS=-halt-on-error -shell-escape

$(CONTENT).pdf: $(ALLTEXFILES) $(ALLFIGS) $(BIBLIOGRAPHY)
	pdflatex $(LATEX_ARGS) $(CONTENT)
	bibtex $(CONTENT)
	pdflatex $(LATEX_ARGS) $(CONTENT)
	pdflatex $(LATEX_ARGS) $(CONTENT)

$(CONTENT)-final.pdf: $(CONTENT).pdf
	gs -sDEVICE=pdfwrite -o $@ \
		-dPDFSETTINGS=/prepress \
		-dDownsampleColorImages=true \
		-dDownsampleGrayImages=true \
		-dDownsampleMonoImages=true \
		-dColorImageResolution=600 \
		-dDoThumbnails=false \
		-f $^

summary_of_changes.pdf: summary_of_changes.md
	pandoc $^ -o $@

.PHONY: paper
paper: $(CONTENT).pdf

.PHONY: final
final: $(CONTENT)-final.pdf

.PHONY: update_check
update_check:
	mkdir -p ./scripts/
	wget https://raw.githubusercontent.com/erich666/chex_latex/master/chex_latex.pl \
		-O ./scripts/chex_latex.pl

.PHONY: check
check:
	perl ./scripts/chex_latex.pl $(ALLTEXFILES)

.PHONY: clean
clean:
	rm -f *.aux *.bbl *.blg *.dvi *.lbl *.log $(CONTENT).pdf \
		$(CONTENT)-final.pdf *.ps *.brf summary_of_changes.pdf


